Synthesis of coordination programs from linear temporal logic

This paper presents a method for synthesizing a reactive program which coordinates the actions of a group of other reactive programs, so that the combined system satisfies a temporal specification of its desired long-term behavior. Traditionally, reactive synthesis has been applied to the construction of a stateful hardware circuit. This work is motivated by applications to other domains, such as the IoT (the Internet of Things) and robotics, where it is necessary to coordinate the actions of multiple sensors, devices, and robots. The mathematical model represents such entities as individual processes in Hoare's CSP model. Given a network of interacting entities, called an \emph{environment}, and a temporal specification of long-term behavior, the synthesis method constructs a \emph{coordinator} process (if one exists) that guides the actions of the environment entities so that the combined system is deadlock-free and satisfies the given specification. The main technical challenge is that a coordinator may have only \emph{partial knowledge} of the environment state, due to non-determinism within the environment, and environment actions that are hidden from the coordinator. This is the first method to handle both sources of partial knowledge, and to do so for arbitrary linear temporal logic specifications. It is shown that the coordination synthesis problem is \PSPACE-hard in the size of the environment. A prototype implementation is able to synthesize compact solutions for a number of coordination problems.

==> Section/intro2.tex <==
\section{Introduction}
\label{Sec:Intro}
%In several settings, it is necessary to coordinate the behavior of a number of independent entities in order to meet a common goal. Consider, for instance, the operation of a so-called ``smart building,'' where
%readings from multiple sensors should be linked to the actions of heating and cooling devices to constantly maintain a proper  temperature and humidity. The
%a control program must regularly monitor various sensors, keep track of the state of the heating and cooling devices, and be able to react to unexpected events such as sensor or device failures. 

Coordinated multi-agent systems are seeing increased adoption  to achieve complex tasks. These tasks may range from maintaining ambient conditions in domestic-purpose smart buildings, where various sensors must be monitored regularly in order to to keep track of the state of the heating and cooling devices, to industrial warehouses with a group of package-carrying robots where one should be
able react to unexpected robot failures and behaviors.  
Typically in these settings, the individual agents are {reactive} and a {centralized coordinator} interacts with them  in order to achieve the task. 
Since the onus of achieving the task largely lies on the  centralized coordinator, it is important to  design a {\em provably correct coordinator}.
Therefore, this work looks into the problem of  automated construction of a  coordinator, or a {\em coordination program}, from a {\em specification} of the desired behavior of the coordinated system. 

%This paper explores the extent to which such reactive coordination programs can be generated fully automatically from a specification of the desired system behavior expressed in linear temporal logic. Temporal synthesis methods have a long history --- it was Alonzo Church who, in 1957, originated the question of synthesizing a stateful hardware circuit from a temporal specification~\cite{church57,church62}. Subsequent breakthroughs by B\"uchi and Landweber~\cite{buechi-landweber69}, Rabin~\cite{rabin69}, and many others have established firm theoretical foundations based on logic, automata and game theory. 



{\em Coordination synthesis} is a particularly attractive option as the challenge of manually designing reactive coordinators is aggravated as the coordinator may only have {\em partial knowledge} of the global state of the system. Partial knowledge of the global system is easily manifested in coordinating systems due to the presence of concurrency, asynchrony, distribution, and so on. In coordinating systems, it may also arise from {\em internal private interactions} among individual devices that do not even interface with the coordinator. 
%due to the presence of concurrency, asynchrony, distribution and so on. A common manifestation of these features is that the coordinator may have to operate with {\em partial knowledge} of the global state of the system, and still ensure that the goal is achieved. Another source of partial knowledge are private interactions among individual devices that may not even interface with the coordinator. 
%For example, consider a warehouse with multiple reactive robots where the objective is to ensure that every package is delivered only after it is packed. Here, the coordinator may be able to interface with the robots when the package is packed and when it is delivered. It may not know whether the package is securely packed. 
%For example, the packing and delivering robots may interact among themselves to deliver only 10 packages at a time, as opposed to delivering each package as it arrives. 
By shifting from an imperative to declarative paradigm of programming/reasoning, coordination synthesis holds the promise to improve the experience of designing a coordination program as it allows the programmer to only focus on the high-level objectives and not on the trickier and error-prone low-level details arising from reactiveness and partial knowledge, among others.  


% What makes synthesis particularly attractive in a coordinating multi-agent system is that as there is considerable variety in coordination scenarios: new devices may be added over time, devices have diverse functionalities, while existing ones may fail unpredictably. The ``how" is usually customized to an installation. This variability makes it infeasible to write a single generic coordination program, and unattractive to re-program coordination by hand after every change. Whereas, customization of the ``what''  is typically much easier. 

Although this work coins the term ``coordination synthesis'', the problem to synthesize centralized reactive coordinators has been addressed before.
However, so far prior work has been able to straddle only one of two objectives of coordination synthesis:  the ability to work with partial knowledge or rich expressiveness of specifications.  
The core contribution of this work is to develop a framework for coordination synthesis that accomplishes both objectives - addresses partial knowledge as well as permits rich expressiveness of specifications.
 
Elaborating further, existing work on coordination synthesis 
can be broadly classified into {\em synchronous synthesis} and {\em asynchronous synthesis}. 
The bulk of existing literature is on synchronous synthesis~\cite{church57,church62,buechi-landweber69,rabin69,pnueli1989synchsynthesis,kupferman2005safraless,bohy2012acacia+,bloem2012synthesis, schewe2013bounded-journal,alur2016compositional,hadaz2018reactive}.
Here, the specifications can be written in highly expressive forms, such as temporal logics, regular expressions, automata and the like. 
But they make the critical assumption that the coordinator must have {\em complete knowledge} of the local states of all the reactive agents at all times.
On the contrary, {\em asynchronous synthesis} incorporates notions of partial knowledge in the coordination program. 
However, it pays for the price of partial knowledge by lowering the  expressiveness of specifications. For example, in Pnueli and Rosner's  seminal work on asynchronous synthesis~\cite{pnueli1989synthesis}, the coordinating program may only sample the input stream from other agents at arbitrary times.  Even very basic specifications such as copying an input stream to the output stream has no solution in this model. More recent work on asynchronous synthesis with a CSP  model, described in detail below, has been able to extend the expressiveness to simple assume-guarantee-like temporal specifications~\cite{d2013synthesizing}. 
 


\begin{figure}[t]
	\begin{center}
		%    \includegraphics[scale=0.45]{system2.pdf}
		\includegraphics[scale=0.45]{Figures/system2.png}
	\end{center}
	\caption{The coordination model. The coordinator $M$ may communicate with the entities $\{E_i\}$ only through a public interface (shown as solid green lines); it need not have a direct link to every entity. Private interactions between the entities (shown as dashed red lines) are hidden from the coordinator. The specification $\varphi$, however, is ``all-seeing'' -- it may refer to private as well as public events.}
	\label{fig:system}
\end{figure}


This brings us to the {\em first contribution} of this work. We present a new formulation of the coordination synthesis problem. In our formulation,  reactive agents and  the to-be-synthesized coordination program are modeled as Communicating Sequential Processes (CSP) 
~\cite{DBLP:journals/cacm/Hoare78,DBLP:books/ph/Hoare85}, whereas specifications are expressed in Linear Temporal Logic (LTL)~\cite{pnueli1977temporal}. 

We choose CSPs for our formulation since in addition to being  mathematically well-defined, they capture the complexities of interactions and partial information in coordinating systems very well (see Fig.~\ref{fig:system}). Each CSP process (reactive agent and coordinator) has a set of {\em public actions}, with which it interacts with other processes, and a set of {\em private actions}, which are hidden from all other processes in the system. Each CSP process may evolve its state by taking a private action without informing any other process in the system. In particular, since these actions are hidden from the coordinator, private actions introduce one level of partial knowledge in coordination. There is further granularity in the {\em public actions} as well.  When two CSP processes interact with each other through a public action, they may do it {\em internally} without informing other CSP processes. In particular, internal interactions among reactive agents may not be observed by the coordinator, introducing yet another level of partial information. 
Finally, processes may be {\em non-deterministic} (due to abstraction) i.e. a process may evolve to more than one state on a public or private interaction. This introduces a third level of partial information. 

Together, these three forms of partial information encompass a large class of coordinating systems, including IoT devices, heterogeneous systems of robots etc. 

In our problem formulation, we allow the LTL specification to be defined on the public and private actions of all CSPs, irrespective of whether they are visible to the coordinator or not. 
It is worth noting that the specification is ``all-seeing'' and can refer to every action; for example, it may include a fairness assumption that rules out an infinite self-loop on an internal interaction. 

Therefore, our {\em coordination synthesis problem} is stated as follows:
Given $n$-CSP processes $E_1,\dots E_n$, referring to the $n$-reactive agents, and an LTL specification $\varphi$ over their public and private actions, does their exist a CSP process $M$, referring to the coordination program such that all  interactions of $E_1\cdot E_n$ and $M$, denoted by $E_1 \choice \dots \choice E_n \choice M$ satisfy the specification $\varphi$? If yes, then construct $M$.





%\paragraph{Motivation.} 
%This work is motivated by potential uses of temporal synthesis in domains other than hardware: in particular, for applications such as the  control of a diverse collection of IoT (Internet of Things) sensors and actuators, and the management of a heterogeneous group of robots. These tasks are reactive and long-running: the controller for a smart building should ideally run forever -- termination is a serious error! Temporal logic is well-suited to describing such long-term behavior.



		
%		We therefore suggest a different, more expressive model for the purpose, based on the well studied framework of Communicating Sequential Processes (CSP) introduced by Hoare~\cite{DBLP:journals/cacm/Hoare78,DBLP:books/ph/Hoare85}. Known entities (devices, sensors, robots) are modeled mathematically as CSP processes: each is a state machine with a set of associated interface actions. The coordinator is also a process of the same type. The model is sketched in Figure~\ref{fig:system}. In CSP,  processes communicate only through an instantaneous, synchronized interaction on a common action: if process $P$ may evolve to process $P'$ on action $a$ and process $Q$ may evolve to $Q'$ on $a$, the concurrent composition $P\parallel Q$ may \emph{jointly} evolve to $P'\parallel Q'$ on event $a$. On the other hand, a process may also have internal actions, which are unsynchronized. We show (in the Appendix) that the CSP model subsumes both the synchronous and the asynchronous synthesis models. 
		
		%The CSP model thus provides a mix of synchronized and asynchronous events It is also well-suited to implementation; for instance, in the programming language \textsf{Go}~\cite{golang}, which implements the CSP model. 
		
		%: as shown in Figure~\ref{fig:system}, the coordinator communicates with each device entity through synchronized actions on their interface. For the example discussed previously, a coordinator may determine the illumination level by synchronizing with the illumination sensor on an action, say \textsf{lowLight}, and turn on a lamp by synchronizing on an action, say \textsf{switchOn}, with the process representing the lamp. 
		
		%\paragraph{Technical Contributions.}
		%The coordination synthesis task can now be stated as the following: given an \emph{environment} CSP process, $E$, representing the joint behavior of a group of CSP processes, and a specification, $\varphi$, of the desired long-term system behavior expressed in linear temporal logic (LTL), construct a CSP process $M$, the \emph{coordinator}, (if one exists) such that the combined system, $E\parallel M$, is (1) free of deadlock, and (2) satisfies $\varphi$ on each of its infinite executions. 
		
		%This formulation makes two implicit choices. The first is to synthesize a single, central coordinator rather than a distributed one. This is acceptable for many coordination scenarios in motivating domains of IoT and robotics; moreover, the synthesis of fully distributed coordination is undecidable in most cases~\cite{pnueli-rosner-1990}. The second choice is to have a single process $E$ represent the behavior of a group of entities. This could be limiting for large enough groups, but the current algorithm is focused on solving other challenges. Ameliorating state explosion in $E$ arising from a large number of entities will require new, modular synthesis methods to be developed. 
		
		%Our main technical contribution is an algorithm to solve the coordination synthesis problem.  The key challenge is that a coordinator may have only partial knowledge of the current environment state. This can arise in two ways. First, the environment model may (due to abstraction) have a non-deterministic response to an interaction at its public interface. Second, the environment entities may have internal interactions that are necessarily hidden from any coordinator. The result is that, from a coordinator's point of view, the environment may be in any one of a \emph{set} of states  after a series of interactions. The future actions of the coordinator must be such that the resulting behavior is correct regardless of the actual state of the environment. 
		
		
		The {\em second contribution}  of this work is an algorithm to solve the coordination synthesis.
		To the best of our knowledge, the algorithm developed in this work is the first to take all three sources of partial information into account, and to do so for the full LTL specification logic. 
		The most closely related work is~\cite{d2013synthesizing} (mentioned earlier) that also uses CSPs but permits partial information only  through non-determinism  only. Private actions and internal interactions are disallowed.  
		In addition, the specifications in~\cite{d2013synthesizing} are limited to GR(1), a strict subset of LTL. (An in-depth discussion of related work appears later in this paper.)
		
		
		The central result here is that coordination synthesis reduces to synchronous synthesis of a new regular specification i.e. the specification can be represented by an automaton. This automaton, called the {\em specification automaton}, combines the behavior of the reactive agents $E_1\dots E_n$ and automaton $\mathcal{A}$ for the LTL specification $\varphi$.
		The key challenge in construction of the specification automaton is to mitigate partial information.
		Naive methods to eradicate partial information employ subset-construction based methods, resulting in a specification automaton with an exponential number of states in the number of states in all reactive agents $E_i$. To avoid this expensive blow-up, we provide an alternate construction of the specification automaton that utilizes {\em transitive closures} only. As a result, the number of states in our specification automaton is only {\em linear} in the number of states of $E_i$s. A drawback of our transitive closure based construction is that the transition relation of the specification automaton has size \emph{exponential} in the number of public (i.e., interface) actions of the environment $E$. However, the   exponential blowup of the transition relation can be ameliorated in implementations by use of symbolic constructions. 
		
		%The core of the algorithm is a new automaton construction which combines the behavior of the environment, $E$, with an automaton, $\mathcal{A}$ for the LTL specification $\varphi$. This construction encodes both types of partial information, representing interface non-determinism through non-deterministic choice, and abstracting from hidden events via a closure construction. The result is a new automaton, $\mathcal{B}$, with a new alphabet and the property that any finite-state machine satisfying $\mathcal{B}$ represents a coordinator process for the original problem. The number of states in $\mathcal{B}$ is \emph{linear} in the number of states of $\mathcal{A}$ and those of $E$; however, its transition relation has size \emph{exponential} in the number of public (i.e., interface) actions of the environment $E$.
		
		For a well-rounded understanding of coordination synthesis, we also conduct a  complexity theoretic   analysis. We prove that coordination synthesis is \PSPACE-hard in the size of the reactive agents $E_1 \cdots  E_n$ for a fixed specification; for comparison, model-checking is in \NLOGSPACE. The hardness result  is not unexpected since problems in reactive synthesis typically exhibit high complexity. For instance, synchronous and asynchronous synthesis for LTL specifications, which are both subsumed by our model (see Appendix), are already \TWOEXPTIME-complete in the size of the specification~\cite{pnueli1989synchsynthesis,pnueli1989synthesis}.
		
		
		In the final part of this work, we present a prototype implementation of our algorithm, replete with the symbolic construction of the central reduction using Binary Decision Diagrams (BDD)~\cite{bryant1986graph} and state-of-the art tool BoSy~\cite{FFRT17} for synchronous synthesis. We conduct case studies to synthesizes a smart thermostat and arbiters for concurrent processes. Our case studies illustrate how coordination synthesis improve the experience to write/design coordination programs, and also illustrate the flexibility of our model to ensure fairness in concurrent systems. 
		While our prototype implementation has limited scalability currently, our empirical analysis reveals that the prime scalability bottleneck are the back-end tools for synchronous synthesis, indicating that our coordination synthesis tool will benefit from improvements in the already emerging area of reactive synthesis for synchronous systems. 
		These results are encouraging as they show the promise of our coordination synthesis framework, and is a stepping stone to synthesizing complex coordination program for realistic settings. 
		
		%We present an implementation of this method, which has successfully synthesized solutions to several coordination problems. Our implementation constructs $\mathcal{B}$ entirely in symbolic form, using Binary Decision Diagram (BDD) representations to ameliorate the exponential blowup of the transition relation. This automaton is in a format that allows a number of tools for synchronous synthesis to be applied; a synthesized machine is mapped back to a CSP description for $M$. Experiments show that scalability is restricted, however; primarily due to the limitations of the back-end synthesis tools. 
		
		
		%We also show (in the Appendix) that our CSP model subsumes both the synchronous and the asynchronous synthesis models. 
		%\begin{enumerate}
		%\item CSP for reactive agents. and LTL for specifictaions. 
		%\item CSP captures complexities -- partiral information. agents interacting with each other. Internal actions -- no interaction wiht anyone. 
		%\item LTL is very expressive. -- Can be in terms of internal private actions as well. (See figure)
		
		%\item Different from Pieterman as that doesn't take into account internal actions. Spec is GR(1) strict fragment of LTL. Since model doesn't even have internal actions, spec does not have them naturally.
		%\item Also, subsumes models of synchrony and asynchrony.  
		%\item envison these kinds of problems being solved with this. 
		%	\item Hardness of coordination synthesis. 
		%\end{enumerate}
		
		
		
	
	%	\paragraph{Summary of contributions.} This work defines and provides a solution for a new form of reactive program synthesis: that of constructing a program that coordinates the actions of a group of other mutually interacting programs, so that the combined system meets a given temporal specification. A first contribution is in formulating a CSP-based model for the problem, as existing models turn out to be inadequate. The second contribution is in the solution method, which is the first (to the best of our knowledge) to fully handle partial information, and do so for arbitrary LTL specifications. This method has been implemented and used to successfully synthesize solutions to several coordination problems. We show, however, that there are practical and complexity-theoretic limitations to scalability, which suggests new research directions in approximate methods for synthesis.
		
		% context
		% ambitious
		
		
		
		
		


==> Section/intro3.tex <==
\section{Introduction}
\label{Sec:Intro}
%In several settings, it is necessary to coordinate the behavior of a number of independent entities in order to meet a common goal. Consider, for instance, the operation of a so-called ``smart building,'' where
%readings from multiple sensors should be linked to the actions of heating and cooling devices to constantly maintain a proper  temperature and humidity. The
%a control program must regularly monitor various sensors, keep track of the state of the heating and cooling devices, and be able to react to unexpected events such as sensor or device failures. 

The task of coordinating the behavior of multiple independent agents in order to meet a common goal arises in several domains. Consider for instance, the Internet of Things (IoT) domain. In a so-called ``smart'' building, various sensors and heating and cooling devices must work in concert to maintain comfortable conditions. In automated multi-robot factories, a number of robots with different capabilities collaborate to carry out various tasks. Another example is from the domain of web services where, for instance, airline, train and hotel services must be queried to book a family vacation.

Typically the individual agents are {reactive} and a {centralized coordinator} guides them in order to carry out a task. As the onus of achieving the task largely lies on the coordinator, it is important to  design a {\em provably correct} coordinator. The construction of coordinators is complicated by several factors, among the main ones are concurrency, asynchrony and distribution, all of which contribute to a coordinator having only \emph{partial knowledge} of the global state of the system. In addition, a coordinator may be required to recover gracefully from agent failures, and (especially in robotics applications) correctly handle noisy data.

Although the design of a coordinator is complex, it is often the case that the task it must achieve can be easily specified. In this work, we therefore consider the question of automatically constructing a reactive coordination 
program from a description of the available agents and a specification of the desired behavior of the properly coordinated system.

The promise of automated synthesis is that it can significantly improve the design experience, as it allows a programmer to focus on  high-level objectives and not on the trickier and error-prone low-level implementation details. On the other hand, synthesis is a highly challenging task, not to be suggested lightly. In coordination settings, one often observes that although the internal structure of an agent may be complex, its external interface is significantly simpler---and it is only the interface behavior that matters for coordination.

For instance, consider the following simple scenario. We have available an illumination sensor, a clock, a number of decorative outdoor lamps, and a timer, and would like to light up the lamps for, say, two hours after dusk. The task is easily described in temporal logic. For this coordination problem, it suffices to model each device as a small, abstract finite state machine. The illumination sensor model may have only two states, low and high; the clock model needs to be accurate only to the hour, and the timer model can have a similar coarse granularity; while each lamp is modeled as being either on or off. A reactive coordination program for this task would check the illumination sensor and the clock to determine when it is dusk, switch on the lamps and set the timer for two hours, switch off the lamps once the timer expires, and repeat the cycle the following day.

%This paper explores the extent to which such reactive coordination programs can be generated fully automatically from a specification of the desired system behavior expressed in linear temporal logic. Temporal synthesis methods have a long history --- it was Alonzo Church who, in 1957, originated the question of synthesizing a stateful hardware circuit from a temporal specification~\cite{church57,church62}. Subsequent breakthroughs by B\"uchi and Landweber~\cite{buechi-landweber69}, Rabin~\cite{rabin69}, and many others have established firm theoretical foundations based on logic, automata and game theory. 


% What makes synthesis particularly attractive in a coordinating multi-agent system is that as there is considerable variety in coordination scenarios: new devices may be added over time, devices have diverse functionalities, while existing ones may fail unpredictably. The ``how" is usually customized to an installation. This variability makes it infeasible to write a single generic coordination program, and unattractive to re-program coordination by hand after every change. Whereas, customization of the ``what''  is typically much easier. 

Although this work coins the term ``\emph{coordination synthesis}'' there is prior work on synthesizing reactive coordination programs. The core contributions of this work are an expressive framework for specifying coordination problems, and a new synthesis algorithm that constructs coordinators which operate with partial knowledge of the environment state, while guiding the combined system so that it satisfies a specification from a rich class of temporal properties. 

%% The core contribution of this paper is a framework that permits specification of coordination p
%% However, so far prior work has been able to straddle only one of two objectives of coordination synthesis:  the ability to work with partial knowledge or rich expressiveness of specifications.  
%% The core contribution of this work is to develop a framework for coordination synthesis that accomplishes both objectives - addresses partial knowledge as well as permits rich expressiveness of specifications.

The bulk of the existing literature on reactive synthesis is on methods for \emph{synchronous} models of computation (cf.~\cite{church57,church62,buechi-landweber69,rabin69,pnueli1989synchsynthesis,kupferman2005safraless,bohy2012acacia+,bloem2012synthesis, schewe2013bounded-journal,alur2016compositional,hadaz2018reactive}). This model is not a good match for the types of coordination scenarios described above, simply because those systems are naturally asynchronous: there is no common clock. In the asynchronous model developed by Pnueli and Rosner~\cite{pnueli1989synthesis}, the synthesized program can only sample the state of the environment at times set by an  adversarial schedule. The model is quite weak as a result: even basic specifications such as copying an input stream to the output have no solution.

Recent work~\cite{d2013synthesizing} shows how to synthesize controllers that can handle a particular form of partial knowledge: non-determinism at an agent interface. That algorithm, however, is limited to specifications in a subclass of linear temporal logic called GR(1), while the model does not allow agents to have internal actions or private agent-to-agent interactions, which are a natural feature of many scenarios. Our new framework allows all these forms of interaction, which are hidden from the coordinator,  while the synthesis algorithm applies to specifications expressed as arbitrary LTL formulas or automata. In both respects, this represents a significant expansion of the class of solvable coordination problems.

\begin{figure}[t]
	\begin{center}
		%    \includegraphics[scale=0.45]{system2.pdf}
		\includegraphics[scale=0.45]{Figures/system2.png}
	\end{center}
	\caption{The coordination model. The coordinator $M$ may communicate with the agents $\{E_i\}$ only through a public interface (shown as solid green lines); it need not have a direct link to every agent. Private agent-to-agent interactions between the agents (shown as dashed red lines) are hidden from the coordinator. Internal actions, not shown in the figure, remain inside agents $E_i$. The specification $\varphi$, however, is ``all-seeing'' - it may refer to private as well as public interactions.}
	\label{fig:system}
\end{figure}

The {\em first contribution} of this work is a new formulation of the coordination synthesis problem. In our formulation,  reactive agents and  the to-be-synthesized coordination program are modeled in Hoare's model of Communicating Sequential Processes (CSP)~\cite{DBLP:journals/cacm/Hoare78,DBLP:books/ph/Hoare85}, and specifications are expressed in Linear Temporal Logic (LTL)~\cite{pnueli1977temporal} or as automata. 

We based the coordination model on the extensively studied CSP framework, as it captures the complexities of interaction and partial knowledge in coordinating systems very well (see Fig.~\ref{fig:system}). Each CSP process (an agent or the coordinator) has a set of {\em public actions}, with which it interacts with other processes, and a set of {\em private actions}, which are hidden from all other processes in the system. A CSP process may evolve its state through an {internal action}, i.e. by taking an private action without involving any other process in the system. In particular, as these actions are hidden from the coordinator, such internal actions introduce one form of partial knowledge. Moreover, {private agent-to-agent interactions} are also unobserved by the coordinator, introducing yet another form of partial knowledge. Finally, an interaction of an agent with the coordinator through its public interface could have {non-deterministic} effects (due to abstraction), so that the next state of the agent is unknown to the coordinator. That introduces a third form of partial knowledge.
%This model suffices to describe a large class of coordinating systems, including IoT devices, heterogeneous systems of robots etc.
The classical models for synchronous and asynchronous synthesis, mentioned above, are both subsumed by this model (see Appendices ~\textsection~\ref{Sec:async-sim}-~\ref{Sec:sync-sim}).


Although the coordinator program must operate correctly under partial knowledge, the specification, on the other hand, is ``all-seeing'' and can refer to every action: internal process actions, agent-to-agent interactions, and agent-to-coordinator interactions. For instance, a specification may include a fairness assumption that rules out an infinite self-loop on an internal interaction. 

This discussion leads to the definition of the specific {\em coordination synthesis problem} considered in this work. Given CSP processes $E_1, \ldots, E_n$, each modeling a reactive agent, and a temporal 
specification $\varphi$ over their public and private actions, construct a CSP process $M$, such that the combined system, denoted $E \parallel M$ (where $E=E_1 \parallel E_2 \parallel \ldots \parallel E_n$), satisfies the specification $\varphi$. 
%
We say that the given problem instance is {\em realizable} if such a CSP process
$M$ exists, otherwise, the given problem instance is {\em unrealizable}.
%
%{\em realizability} amounts to checking whether there exist a CSP process $M$,
%such that all of its interactions of $E_1,\ldots E_n$ satisfy specification
%$\varphi$; If is realizables, {\em synthesis} construct $M$.
%
% does their exist
% a CSP process $M$, referring to the coordination program such that all
% interactions of $E_1\ldots E_n$ and $M$ satisfy the specification $\varphi$? If
% yes, then construct $M$.
%


%\paragraph{Motivation.} 
%This work is motivated by potential uses of temporal synthesis in domains other than hardware: in particular, for applications such as the  control of a diverse collection of IoT (Internet of Things) sensors and actuators, and the management of a heterogeneous group of robots. These tasks are reactive and long-running: the controller for a smart building should ideally run forever -- termination is a serious error! Temporal logic is well-suited to describing such long-term behavior.

%		We therefore suggest a different, more expressive model for the purpose, based on the well studied framework of Communicating Sequential Processes (CSP) introduced by Hoare~\cite{DBLP:journals/cacm/Hoare78,DBLP:books/ph/Hoare85}. Known entities (devices, sensors, robots) are modeled mathematically as CSP processes: each is a state machine with a set of associated interface actions. The coordinator is also a process of the same type. The model is sketched in Figure~\ref{fig:system}. In CSP,  processes communicate only through an instantaneous, synchronized interaction on a common action: if process $P$ may evolve to process $P'$ on action $a$ and process $Q$ may evolve to $Q'$ on $a$, the concurrent composition $P\parallel Q$ may \emph{jointly} evolve to $P'\parallel Q'$ on event $a$. On the other hand, a process may also have internal actions, which are unsynchronized. We show (in the Appendix) that the CSP model subsumes both the synchronous and the asynchronous synthesis models. 
		
%The CSP model thus provides a mix of synchronized and asynchronous events It is also well-suited to implementation; for instance, in the programming language \textsf{Go}~\cite{golang}, which implements the CSP model. 
		
%: as shown in Figure~\ref{fig:system}, the coordinator communicates with each device entity through synchronized actions on their interface. For the example discussed previously, a coordinator may determine the illumination level by synchronizing with the illumination sensor on an action, say \textsf{lowLight}, and turn on a lamp by synchronizing on an action, say \textsf{switchOn}, with the process representing the lamp. 

%\paragraph{Technical Contributions.}
%The coordination synthesis task can now be stated as the following: given an \emph{environment} CSP process, $E$, representing the joint behavior of a group of CSP processes, and a specification, $\varphi$, of the desired long-term system behavior expressed in linear temporal logic (LTL), construct a CSP process $M$, the \emph{coordinator}, (if one exists) such that the combined system, $E\parallel M$, is (1) free of deadlock, and (2) satisfies $\varphi$ on each of its infinite executions. 

%This formulation makes two implicit choices. The first is to synthesize a single, central coordinator rather than a distributed one. This is acceptable for many coordination scenarios in motivating domains of IoT and robotics; moreover, the synthesis of fully distributed coordination is undecidable in most cases~\cite{pnueli-rosner-1990}. The second choice is to have a single process $E$ represent the behavior of a group of entities. This could be limiting for large enough groups, but the current algorithm is focused on solving other challenges. Ameliorating state explosion in $E$ arising from a large number of entities will require new, modular synthesis methods to be developed. 

%Our main technical contribution is an algorithm to solve the coordination synthesis problem.  The key challenge is that a coordinator may have only partial knowledge of the current environment state. This can arise in two ways. First, the environment model may (due to abstraction) have a non-deterministic response to an interaction at its public interface. Second, the environment entities may have internal interactions that are necessarily hidden from any coordinator. The result is that, from a coordinator's point of view, the environment may be in any one of a \emph{set} of states  after a series of interactions. The future actions of the coordinator must be such that the resulting behavior is correct regardless of the actual state of the environment. 
		
		
The {\em second contribution} of this work is an algorithm to solve this problem.
To the best of our knowledge, this is the first algorithm that takes all three sources of partial knowledge into
account, and does so for arbitrary LTL specifications. (An in-depth
discussion of related work appears later in this paper.) We reduce coordination
synthesis to the ordinary synthesis of a new temporal specification which can be
represented as an automaton. This automaton, called the {\em specification
automaton}, combines the behavior of the reactive agents $E_1,\ldots,E_n$, 
in an asynchronous setting, with an automaton $\mathcal{A}$ for the LTL specification $\varphi$.

The key challenge in this construction is to represent the partial knowledge of
the environment state. A naive encoding would use a subset
construction, producing an exponential blowup in the number of states of $E$.
We provide an alternate construction, where the number of states in our specification automaton grows \emph{linearly} with the number of states of $E$
and the number of states of the property automaton $\mathcal{A}$. 
Although the number of states grows linearly, the transition relation of the 
specification automaton has size exponential in the number of public
actions (i.e., interface) of the environment $E$. 
%
To ameliorate the exponential blowup incurred by the transition relation we use
symbolic constructions.
%
% However, the exponential
% blowup of the transition relation can be ameliorated in implementations by use
% of symbolic constructions, which we provide and also implement.



%The core of the algorithm is a new automaton construction which combines the behavior of the environment, $E$, with an automaton, $\mathcal{A}$ for the LTL specification $\varphi$. This construction encodes both types of partial knowledge, representing interface non-determinism through non-deterministic choice, and abstracting from hidden events via a closure construction. The result is a new automaton, $\mathcal{B}$, with a new alphabet and the property that any finite-state machine satisfying $\mathcal{B}$ represents a coordinator process for the original problem. The number of states in $\mathcal{B}$ is \emph{linear} in the number of states of $\mathcal{A}$ and those of $E$; however, its transition relation has size \emph{exponential} in the number of public (i.e., interface) actions of the environment $E$.

		
Towards a full understanding of the inherent difficulty of coordination
synthesis,  
our {\em third contribution} is to
prove a complexity-theoretic result showing that the question is
\PSPACE-hard in the size of $E$ for a fixed specification; in comparison,
model-checking is in \NLOGSPACE. This rather severe hardness result is not
entirely unexpected since problems in reactive synthesis typically exhibit high
worst-case complexity. For instance, both synchronous and asynchronous synthesis
for 
arbitrary LTL specifications are known to be \TWOEXPTIME-complete in the size
of the specification~\cite{pnueli1989synchsynthesis,pnueli1989synthesis}.
		
We also present a prototype implementation of our algorithm, which uses a
symbolic construction of the specification automaton, using Ordered Binary Decision
Diagrams (BDDs)~\cite{bryant1986graph}, and relies on the state-of-the-art tool
BoSy~\cite{FFRT17} for the final ordinary synthesis step. We present case
studies on synthesizing a smart thermostat, and arbiters for concurrent
processes. Our case studies illustrate the capabilities of the model, and show
how synthesis improves the experience of designing coordination
programs. While this prototype has limited scalability, additional
empirical analysis reveals that the primary bottleneck is in the current capabilities of the back-end synthesis tools.
Improvements to these tools (an active research topic) will therefore have a positive effect on the scalability of coordination synthesis.
The most impressive impact on scalability is, however, likely to come from entirely new synthesis methods which exploit symmetry, modularity, and abstraction,
drawing inspiration from the success of such techniques in formal verification. % can be expected to have an even greater impact on scalability. 
%\yssnote{the modularity sentance should come here\ldots}

%%results as s are encouraging as they show romise of our coordination synthesis framework, and is a stepping stone to synthesizing complex coordination program for realistic settings. 
		
%We present an implementation of this method, which has successfully synthesized solutions to several coordination problems. Our implementation constructs $\mathcal{B}$ entirely in symbolic form, using Binary Decision Diagram (BDD) representations to ameliorate the exponential blowup of the transition relation. This automaton is in a format that allows a number of tools for synchronous synthesis to be applied; a synthesized machine is mapped back to a CSP description for $M$. Experiments show that scalability is restricted, however; primarily due to the limitations of the back-end synthesis tools. 
		
		
%We also show (in the Appendix) that our CSP model subsumes both the synchronous and the asynchronous synthesis models. 
%\begin{enumerate}
%\item CSP for reactive agents. and LTL for specifictaions. 
%\item CSP captures complexities -- partiral knowledge. agents interacting with each other. Internal actions -- no interaction wiht anyone. 
%\item LTL is very expressive. -- Can be in terms of internal private actions as well. (See figure)
		
%\item Different from Pieterman as that doesn't take into account internal actions. Spec is GR(1) strict fragment of LTL. Since model doesn't even have internal actions, spec does not have them naturally.
%\item Also, subsumes models of synchrony and asynchrony.  
%\item envison these kinds of problems being solved with this. 
%	\item Hardness of coordination synthesis. 
%\end{enumerate}
		
		
		
	
\paragraph{Summary of contributions.} This work defines and provides a solution
for a new form of reactive program synthesis: that of constructing a program
that coordinates the actions of a group of other mutually interacting programs,
so that the combined system meets a given temporal specification. A first
contribution is in formulating an expressive CSP-based model for the problem, as
existing models turn out to be inadequate. The second contribution is in the
solution method, which is the first (to the best of our knowledge) to fully
handle partial knowledge, and do so for arbitrary LTL specifications. 
The third contribution is a complexity theoretic analysis of the coordination synthesis problem. 
The new algorithm has been implemented and used to successfully synthesize solutions to
several coordination problems. We show, however, that there are practical and
complexity-theoretic limitations to scalability, which suggest new research
directions, such as modular methods for synthesis.
%\yssnote{add third contrib (complexity)}

		
		
		
		
		


==> Section/introduction.tex <==

\section{Introduction}
In several settings, it is necessary to coordinate the behavior of a number of independent entities in order to meet a common goal. Consider, for instance, the operation of a so-called ``smart building,'' where
% readings from multiple sensors should be linked to the actions of heating and cooling devices to constantly maintain a proper  temperature and humidity. The
a control program must regularly monitor various sensors, keep track of the state of the heating and cooling devices, and be able to react to unexpected events such as sensor or device failures. The design of such programs can be quite challenging, as a programmer is faced with a number of difficult issues such as concurrency, distribution, partial knowledge of the system state, and the need to gracefully handle noise and failures. 

This paper explores the extent to which such reactive coordination programs can be generated fully automatically from a specification of the desired system behavior expressed in linear temporal logic. Temporal synthesis methods have a long history --- it was Alonzo Church who, in 1957, originated the question of synthesizing a stateful hardware circuit from a temporal specification~\cite{church57,church62}. Subsequent breakthroughs by B\"uchi and Landweber~\cite{buechi-landweber69}, Rabin~\cite{rabin69}, and many others have established firm theoretical foundations based on logic, automata and game theory. 

\paragraph{Motivation.} 
This work is motivated by potential uses of temporal synthesis in domains other than hardware: in particular, for applications such as the  control of a diverse collection of IoT (Internet of Things) sensors and actuators, and the management of a heterogeneous group of robots. These tasks are reactive and long-running: the controller for a smart building should ideally run forever -- termination is a serious error! Temporal logic is well-suited to describing such long-term behavior.

Synthesis is attractive in these domains as there is considerable variety in coordination scenarios: devices have diverse functionalities, new devices may be added over time, while existing ones may fail unpredictably. The specification is usually customized to an installation and may itself change over time. This variability makes it infeasible to write a single generic coordination program, and unattractive to re-program coordination by hand after every change.

Consider the following simple scenario. We have available an illumination sensor, a clock, a number of decorative outdoor lamps, and a timer, and would like to light up the lamps for, say, two hours after dusk. The task is easily described in temporal logic. A program for this task must check the illumination sensor and the clock to determine when it is dusk, switch on the lamps and set the timer for two hours, switch off the lamps once the timer expires, and repeat the cycle the following day. Automatically synthesizing such reactive coordination is the goal of this work.

Program synthesis should not be suggested lightly, as it is an extremely challenging task, in practice and in theory. An encouraging observation in this regard is that the behavior of an individual device can often be abstracted to a small finite state machine. For the scenario above, a model of the illumination sensor may have only two states, low and high; the clock model needs to be accurate only to the hour, and the timer model can have a similar coarse granularity; while each lamp is modeled as being either on or off. 

Coordination synthesis requires a new formulation, however, as existing models for temporal synthesis are inadequate for the purpose. There are two primary models. The classical model considered by Church and others is purely synchronous and is based on low-level read and write actions: at each clock tick, the program to be synthesized reads an input and writes an output value. This is not a good match, as devices and robots operate asynchronously, with interface actions of higher granularity (e.g., \textsf{switchOff} a lamp). The alternative, introduced by Pnueli and Rosner in~\cite{pnueli1989synthesis}, is purely asynchronous: the program to be synthesized may only \emph{sample} a subsequence of an input stream (at adversarially chosen points) and must base its output only on the sample. Basic specifications such as copying an input stream to the output stream have no solution in this model, as shown in the same paper. Neither model is therefore a good fit: one is too strong, the other too weak.


\begin{figure}
  \begin{center}
    %    \includegraphics[scale=0.45]{system2.pdf}
    \includegraphics[scale=0.45]{Figures/system2.png}
  \end{center}
  \caption{The coordination model. The coordinator $M$ may communicate with the entities $\{E_i\}$ only through a public interface (shown as solid green lines); it need not have a direct link to every entity. Private interactions between the entities (shown as dashed red lines) are hidden from the coordinator. The specification $\varphi$, however, is ``all-seeing'' -- it may refer to private as well as public events.}
  \label{fig:system}
\end{figure}

We therefore suggest a different, more expressive model for the purpose, based on the well studied framework of Communicating Sequential Processes (CSP) introduced by Hoare~\cite{DBLP:journals/cacm/Hoare78,DBLP:books/ph/Hoare85}. Known entities (devices, sensors, robots) are modeled mathematically as CSP processes: each is a state machine with a set of associated interface actions. The coordinator is also a process of the same type. The model is sketched in Figure~\ref{fig:system}. In CSP,  processes communicate only through an instantaneous, synchronized interaction on a common action: if process $P$ may evolve to process $P'$ on action $a$ and process $Q$ may evolve to $Q'$ on $a$, the concurrent composition $P\parallel Q$ may \emph{jointly} evolve to $P'\parallel Q'$ on event $a$. On the other hand, a process may also have internal actions, which are unsynchronized. We show (in the Appendix) that the CSP model subsumes both the synchronous and the asynchronous synthesis models. 

%The CSP model thus provides a mix of synchronized and asynchronous events It is also well-suited to implementation; for instance, in the programming language \textsf{Go}~\cite{golang}, which implements the CSP model. 

%: as shown in Figure~\ref{fig:system}, the coordinator communicates with each device entity through synchronized actions on their interface. For the example discussed previously, a coordinator may determine the illumination level by synchronizing with the illumination sensor on an action, say \textsf{lowLight}, and turn on a lamp by synchronizing on an action, say \textsf{switchOn}, with the process representing the lamp. 

\paragraph{Technical Contributions.}
The coordination synthesis task can now be stated as the following: given an \emph{environment} CSP process, $E$, representing the joint behavior of a group of CSP processes, and a specification, $\varphi$, of the desired long-term system behavior expressed in linear temporal logic (LTL), construct a CSP process $M$, the \emph{coordinator}, (if one exists) such that the combined system, $E\parallel M$, is (1) free of deadlock, and (2) satisfies $\varphi$ on each of its infinite executions. 

This formulation makes two implicit choices. The first is to synthesize a single, central coordinator rather than a distributed one. This is acceptable for many coordination scenarios in motivating domains of IoT and robotics; moreover, the synthesis of fully distributed coordination is undecidable in most cases~\cite{pnueli-rosner-1990}. The second choice is to have a single process $E$ represent the behavior of a group of entities. This could be limiting for large enough groups, but the current algorithm is focused on solving other challenges. Ameliorating state explosion in $E$ arising from a large number of entities will require new, modular synthesis methods to be developed. 

Our main technical contribution is an algorithm to solve the coordination synthesis problem.  The key challenge is that a coordinator may have only partial knowledge of the current environment state. This can arise in two ways. First, the environment model may (due to abstraction) have a non-deterministic response to an interaction at its public interface. Second, the environment entities may have internal interactions that are necessarily hidden from any coordinator. The result is that, from a coordinator's point of view, the environment may be in any one of a \emph{set} of states  after a series of interactions. The future actions of the coordinator must be such that the resulting behavior is correct regardless of the actual state of the environment. It is worth noting that the specification is ``all-seeing'' and can refer to every action; for example, it may include a fairness assumption that rules out an infinite self-loop on an internal interaction. 

To the best of our knowledge, the algorithm developed in this work is the first to take both sources of partial information into account, and to do so for the full LTL specification logic. The most closely related work on the CSP model from~\cite{d2013synthesizing} allows interface non-determinism but not internal, hidden events. (An in-depth discussion of related work appears later in this paper.)

The core of the algorithm is a new automaton construction which combines the behavior of the environment, $E$, with an automaton, $\mathcal{A}$ for the LTL specification $\varphi$. This construction encodes both types of partial information, representing interface non-determinism through non-deterministic choice, and abstracting from hidden events via a closure construction. The result is a new automaton, $\mathcal{B}$, with a new alphabet and the property that any finite-state machine satisfying $\mathcal{B}$ represents a coordinator process for the original problem. The number of states in $\mathcal{B}$ is \emph{linear} in the number of states of $\mathcal{A}$ and those of $E$; however, its transition relation has size \emph{exponential} in the number of public (i.e., interface) actions of the environment $E$.

We present an implementation of this method, which has successfully synthesized solutions to several coordination problems. Our implementation constructs $\mathcal{B}$ entirely in symbolic form, using Binary Decision Diagram (BDD) representations to ameliorate the exponential blowup of the transition relation. This automaton is in a format that allows a number of tools for synchronous synthesis to be applied; a synthesized machine is mapped back to a CSP description for $M$. Experiments show that scalability is restricted, however; primarily due to the limitations of the back-end synthesis tools. 

We also show that the coordination synthesis question is \PSPACE-hard in the size of the environment process $E$; for comparison, model-checking is in \NLOGSPACE. (It is well known that the synthesis problem is \TWOEXPTIME-complete in the size of the LTL specification~\cite{pnueli1989synchsynthesis}.)  This complexity result also points to the need for new research on scalable methods to handle large environment processes. 

\paragraph{Summary of contributions.} This work defines and provides a solution for a new form of reactive program synthesis: that of constructing a program that coordinates the actions of a group of other mutually interacting programs, so that the combined system meets a given temporal specification. A first contribution is in formulating a CSP-based model for the problem, as existing models turn out to be inadequate. The second contribution is in the solution method, which is the first (to the best of our knowledge) to fully handle partial information, and do so for arbitrary LTL specifications. This method has been implemented and used to successfully synthesize solutions to several coordination problems. We show, however, that there are practical and complexity-theoretic limitations to scalability, which suggests new research directions in approximate methods for synthesis.

% context
% ambitious




  

